Brain tumor segmentation using synthetic MR images -- A comparison of GANs and diffusion models

Large annotated datasets are required for training deep learning models, but in medical imaging data sharing is often complicated due to ethics, anonymization and data protection legislation. Generative AI models, such as generative adversarial networks (GANs) and diffusion models, can today produce very realistic synthetic images, and can potentially facilitate data sharing. However, in order to share synthetic medical images it must first be demonstrated that they can be used for training different networks with acceptable performance. Here, we therefore comprehensively evaluate four GANs (progressive GAN, StyleGAN 1-3) and a diffusion model for the task of brain tumor segmentation (using two segmentation networks, U-Net and a Swin transformer). Our results show that segmentation networks trained on synthetic images reach Dice scores that are 80% - 90% of Dice scores when training with real images, but that memorization of the training images can be a problem for diffusion models if the original dataset is too small. Our conclusion is that sharing synthetic medical images is a viable option to sharing real images, but that further work is required. The trained generative models and the generated synthetic images are shared on AIDA data hub

==> Reviews.tex <==
Deadline, December 10 ?


Jag tror att man behöver göra det tydligare i tabell 8 hur många som blev klassade rätt eller fel, dvs rubrikerna måste ändras till t ex correct och misclassified.

 

Hur tänker du kring detta att jag har ungefär samma antal klassificerade rätt resp fel i varje kategori? Det är ju inte slump, utan någon typ av systematik i min klassning. Kanske en analys av vilka bilder som jag klassade som real – har de någon liknande egenskap? Vad är det som gör att jag tror att det är just de som är de riktiga?

 

Sen vet jag inte om man ska prata om kvalitet – det kanske är rätt term, men generellt så tycker ju jag att bilderna håller låg kvalitet, dvs de är pixliga och liknar inte alls de kliniska bilder jag är van vid. Men alla bilder håller ungefär samma (låga) nivå, så på det sättet liknar de ju varandra. Det resonemanget tycker jag iofs att vi fångar i diskussionsparagrafen.


List of Experiments 
1. Ratio of Synthetic Data (incremental synthetic data efficiency curve)
2. Transformer Model (Time, Dice Score)


We would like to thank the reviewers for there questions and suggestions which have improved the manuscript.

----

Editorial requests

Are all the output data contained with the details in the paper (figures, tables, text, etc). If there are any machine readable files to validate the results please share these within a suitable repository (https://www.nature.com/sdata/policies/repositories). At present the Data Availability statement only mentions input data - are there any output files?

AE: We have now shared the synthetic images (100,000 five channel images per generative model) and the trained generative models on AIDA data hub, 


Questions : 
**************************************************************
Reviewer # 1 
**************************************************************

1. Although experimental details are provided in section 4.2, more details could be included for the readers to replicate each of the models proposed. Specifically, what are the encoder and decoder structures for each model, if they are altered to fit the needs/resolution requirements of the dataset (or is a default network architecture specified)? What is the scheduler for the diffusion model, what are the training diffusion steps and inference diffusion steps, are they different? Are the learning rate and optimizer specified in section 4.3 also used for the generative models or are a different set of optimizers used?

AE: We answer one question at a time below. The trained generative models have now been shared on AIDA data hub.

What is the scheduler for the diffusion model, what are the training diffusion steps and inference diffusion steps, are they different?

    The "scheduler" in the context of diffusion models generally refers to the way in which noise is added or removed during the diffusion process. The choice of noise schedule can affect the quality of the samples and the efficiency of the model. 

    During training, a diffusion model starts with real data samples, progressively adds noise over several steps according to a predetermined schedule until the data becomes pure noise, and then learns to predict the reverse of this process, reconstructing less noisy data from more noisy data at each step. This iterative procedure trains the model to eventually recreate the original data from noise.

    During inference, a diffusion model initiates with a sample of pure noise and sequentially applies learned denoising steps to reduce the noise, following the reverse of the training noise schedule. This process is iterated until the noise is completely removed, resulting in the generation of a new data sample that resembles the training data distribution.
    
Are the learning rate and optimizer specified in section 4.3 also used for the generative models or are a different set of optimizers used?

    Section 4.3 describes a specific learning rate and optimizer for a UNet used for segmentation, the generative models (GANs, Diffusion Models) used to produce the synthetic images for the segmentation task would likely use a different set of hyperparameters explained in section 4.2. This is because the tasks (segmentation vs. image generation) have different objectives and thus require different training strategies.

    
2. I briefly read through the codebase, and found codes are not released properly, or the documentation is not updated properly. Specifically, the readme of the diffusion model folder gives the command 'python scripts/image_train.py --data_dir datasets/313_3Channel_Images_train/ MODEL_FLAGS DIFFUSION_FLAGS TRAIN_FLAGS', yet file scripts/image_train.py does not exist. Please update the codebase and make sure it is readily usable by others.




3. More experimental results are needed to properly evaluate the quality of the synthetic dataset.
- Tables 3-7 show how the performance would differ when using (i) Original data; (ii) Original+Synthetic data; (iii) Synthetic data. I believe instead of including each type of data in a binary way, it is also critical to see how the amount of the generated synthetic images would affect the performance, and if generating more synthetic images can further help the performance. It would be interesting to show a synthetic data efficiency curve, where the x axis shows different ratios between real/synthetic is used for training, and y axis show the corresponding performance.

    We incrementally increased our dataset with synthetic data alongside real data to train our segmentation model. However, this gradual integration did not yield any significant enhancement in the model's segmentation accuracy. This outcome suggests that the addition of incremental synthetic data, in this case, does not substantially benefit the model's performance.

AE: We should at least mention this in the paper. As the reviewer asks for "more experimental results" we can also mention results from transformer model here.   
    
4. - While I think the qualitative evaluation performed by neuroradiologist is interesting, it is critical to include more details of the evaluation process, and also to include more quantification of the results. Table 8 alone is not intuitive and informative enough to determine the quality of the generated images on itself.

AE: Reply from Ida in Swedish above.    



**************************************************************
Reviewer # 2 
**************************************************************
1. Summarise the results as there are too many tables in the paper 

2. Examples should be provided to justify each of "accuracy, efficiency, and cost-effectiveness".

3. Have evaluations been performed to guarantee that these synthetic data do not contain identifiable patient features?

    In our other work, we have conducted a thorough investigation to ensure that the synthetic data are stripped of any identifiable patient details. This investigation includes the application of various evaluation metrics, such as the Fréchet Inception Distance (FID), Inception Score (IS), and Correlation measures. The detailed findings are accessible in a preprint at the following link: https://arxiv.org/abs/2305.07644
    

4. "Dice similarity coefficient between 1 and 5 percentage points". Dice is not a percentage, so the meaning of this sentence is unclear. (Note: after returning to this comment following a complete readthrough, I suspect the authors mean dice coefficients vary by 1–5\% relative to the baseline performance)

5. Please elaborate upon the content of citations 8 and 17 about why FID and IS may not be strong measures — no need for a deep dive, but added context about what their shortcomings are would help in interpreting the table and relative rankings across measures

    Citations 8 and 17 delve into the specifics of why FID and IS, despite being popular measures for evaluating the perceptual quality of generated images, might not provide a comprehensive picture of the data's utility and privacy. The primary shortcoming of both FID and IS is their focus on the quality and diversity of the generated images, without considering the degree of similarity these images might share with the original training data. In the context of synthetic data meant to replace sensitive real-world data, such as patient images, this is a critical oversight.
  

6. -The transition from testing generative model performance agnostic of segmentation models, Tables 1 and 2, to testing segmentation performance using a combination of original, augmented, and synthetic-only datasets, Tables 3–7, was quite abrupt. It would be better to first summarize the conclusions or insights drawn from Tables 1–2 prior to showing the results for the second phase of the study. The note in Table 2's caption suggests that the conclusion here is that the results of Tables 1 and 2 are unrelated to the following, so perhaps it may be worth saving space and improving clarity by stating this plainly in the text and moving these evaluations to a supplemental section. I would suggest using subsections to separate these sections, while simultaneously providing a clear summary of the relevant findings

7. -Tables 3–7 communicate a large set of performance results, but do so with rather low information density and comparison across tables is quite difficult. Similar to how Table 1 presented a ranked-order of models for various tasks, it could be worth including an equivalent for Tables 3–7, and moving these elements themselves to an appendix.

8. Throughout the results section, tables and figures are enumerated and run through sequentially, with little unpacking or explanation of the implication of the contained results. This paper would be greatly improved with the addition of stronger narrative flow and commentary on the results being presented.
At several points, the authors refer to the relative performance of multiple models with a statement similar to "X is much higher than Y, and we have not yet found any explanation". Given the lack of interpretation or understanding why various models perform better or worse than others, how can readers be expected to apply the knowledge presented in this paper to their own datasets or contexts? For instance, are there particular subjects/samples that are driving variation in performance across these models?

9. A follow-up to the above point is the surprising result that for some tasks, models without augmentation perform best. Is there any rationale for why this may be the case?

10. The definition of the segmentation networks is incomplete until reaching the methods section. It is not clear what model is used here, why it was chosen/constructed, or how different segmentation models may affect the performance and ranking of the synthetic models being compared. Given that the performance on the segmentation task is described and presented as the primary evaluation criteria, these details are important to communicate and rationalize, or compare against alternatives.

11. It appears that Table 7 is the critical result of this manuscript, but given the large number of tables and data presented, this is not immediately clear when reading. Also, is there a reason why no rows have been highlighted in this table to identify the best generative models, as was done elsewhere?

12. Table 8 seems to present percentages, but the caption describes counts. Harmonize?

13. Throughout these results, it is unclear how the sample size for trained models varies across contexts (e.g., Orig + Aug both ticked versus neither ticked), and how that may lead to variations in performance. Please elaborate.

14. the necessary first analysis would be to assess the similarity of synthetic and real data across models using both quantitative and qualitative scoring, and ruling out any generative approaches where clinicians have identified a risk of data memorization.

15. The argument of clinical data/samples being treated as a form of public good, and not requiring further consent for use in research or development, is perhaps a slippery slope and many examples exist where a retrospective look identifies the continued use of such data/samples as an unauthorized abuse (perhaps most famously of Henrieta Lacks). I find this perspective a troubling one to present in a work that is chiefly interested in generating synthetic data, as it seems to undermine the objective of ensuring that adequately anonymous data are produced.








*******************************************************************************************************
Reviewer #1 (Remarks to the Author):

The paper evaluates the quality of the synthetic images produced by generative models for brain tumor segmentation. The authors demonstrated that when training segmentation networks on synthetic images, the networks can reach comparable Dice scores when training with real images. The authors also showed that generative networks, especially diffusion models, contain memorization issues, which could be problematic for applications.

1. \textbf{Experimental details can be more extensive.}
Although experimental details are provided in section 4.2, more details could be included for the readers to replicate each of the models proposed. Specifically, what are the encoder and decoder structures for each model, if they are altered to fit the needs/resolution requirements of the dataset (or is a default network architecture specified)? What is the scheduler for the diffusion model, what are the training diffusion steps and inference diffusion steps, are they different? Are the learning rate and optimizer specified in section 4.3 also used for the generative models or are a different set of optimizers used?

2. \textbf{Error in code documentation.}
I briefly read through the codebase, and found codes are not released properly, or the documentation is not updated properly. Specifically, the readme of the diffusion model folder gives the command 'python scripts/image_train.py --data_dir datasets/313_3Channel_Images_train/ $MODEL_FLAGS $DIFFUSION_FLAGS \$TRAIN_FLAGS', yet file scripts/image_train.py does not exist. Please update the codebase and make sure it is readily usable by others.

3. \textbf{More experimental results are needed to properly evaluate the quality of the synthetic dataset.}
- Tables 3-7 show how the performance would differ when using (i) Original data; (ii) Original+Synthetic data; (iii) Synthetic data. I believe instead of including each type of data in a binary way, it is also critical to see how the amount of the generated synthetic images would affect the performance, and if generating more synthetic images can further help the performance. It would be interesting to show a synthetic data efficiency curve, where the x axis shows different ratios between real/synthetic is used for training, and y axis show the corresponding performance.
- While I think the qualitative evaluation performed by neuroradiologist is interesting, it is critical to include more details of the evaluation process, and also to include more quantification of the results. Table 8 alone is not intuitive and informative enough to determine the quality of the generated images on itself.

Reviewer #2 (Remarks to the Author):

This paper proposes to use synthetic data generating pipelines, GANs in particular, as a means of avoiding issues surrounding privacy and the sharing of private medical data in the context of constructing clinically useful machine learning models, such as for lesion segmentation. This approach tests several GAN architectures and training paradigms (including each combination of real/synthetic and (un)augmented datasets) in their segmentation model, and compares performance across numerous measures. The authors find that segmentation performance can achieve 80–90\% of the performance of using real datasets, and suggest that this could be a viable alternative in contexts when clinical data cannot be shared. In general, I think this is well done work, but I have several concerns regarding the 1) framing of the results, and 2) evaluation of the GAN models and their viability in the presented use case. First, the authors do not compellingly demonstrate that the synthetic datasets are sufficiently distinct from the original data to be considered independent and not from true clinical samples, which directly undermines this approach. While the authors acknowledge that few relevant quantitative measures exist to evaluate synthetic data, they do not satisfyingly tackle this issue or propose how one could define an acceptable range of overlap with true clinical data in order for the risk to be minimized. Conversely, the authors seem to jump past this concern and suggest that GDPR should not apply to synthetic datasets given that they are not derived from any lone individual — while I do not have legal expertise and cannot state the extent to which this is true, by adhering to the spirit of GDPR one would expect that it would be necessary to meet a criteria for producing sufficiently distinct samples than those in the original sample. Second, the authors only evaluate these synthetic datasets using a single segmentation model, which limits the possible generalization of these findings to other models or contexts. This concern is amplified by the authors' own words, in which they regularly state that they do not know why one model or training strategy outperforms another. To overcome this, the authors should compare several segmentation models, and compare how their relative performance varies across training contexts.

Lastly, before providing my more detailed point-by-point notes, below, the results are currently presented with relatively low information density. The organization or results into the current set of tables requires the reader to jump across pages regularly in order to compare the findings in one evaluation to the others, which significantly limits the accessibility and intuitiveness of these results. I would recommend that the authors include each of these extremely detailed and thoroughly populated tables in the appendix, while providing summaries that succinctly capture the take-home messages of each evaluation (similar to the presentation of Table 1).

Overall, I think this work is interesting and well done, and will be of value to the community once the results are demonstrated to both be based on truly non-memorized/repackaged data, and they are shown to generalize and be consistent across segmentation models.

Minor comments:

Introduction:
-Examples should be provided to justify each of "accuracy, efficiency, and cost-effectiveness".
-"A potential solution to facilitate sharing of medical images is therefore to generate and share synthetic images, or more precisely synthetic patients, as GDPR should not apply to medical images which do not belong to a specific person" I believe this requires further unpacking. This statement is true, so long as no potentially descriptive patient-specific features exist within the synthetic images. Have evaluations been performed to guarantee that these synthetic data do not contain identifiable patient features?
-"Dice similarity coefficient between 1 and 5 percentage points". Dice is not a percentage, so the meaning of this sentence is unclear. (Note: after returning to this comment following a complete readthrough, I suspect the authors mean dice coefficients vary by 1–5\% relative to the baseline performance)

Results:
-Please elaborate upon the content of citations 8 and 17 about why FID and IS may not be strong measures ­— no need for a deep dive, but added context about what their shortcomings are would help in interpreting the table and relative rankings across measures.
-The transition from testing generative model performance agnostic of segmentation models, Tables 1 and 2, to testing segmentation performance using a combination of original, augmented, and synthetic-only datasets, Tables 3–7, was quite abrupt. It would be better to first summarize the conclusions or insights drawn from Tables 1–2 prior to showing the results for the second phase of the study. The note in Table 2's caption suggests that the conclusion here is that the results of Tables 1 and 2 are unrelated to the following, so perhaps it may be worth saving space and improving clarity by stating this plainly in the text and moving these evaluations to a supplemental section. I would suggest using subsections to separate these sections, while simultaneously providing a clear summary of the relevant findings.
-Tables 3–7 communicate a large set of performance results, but do so with rather low information density and comparison across tables is quite difficult. Similar to how Table 1 presented a ranked-order of models for various tasks, it could be worth including an equivalent for Tables 3–7, and moving these elements themselves to an appendix.
-Throughout the results section, tables and figures are enumerated and run through sequentially, with little unpacking or explanation of the implication of the contained results. This paper would be greatly improved with the addition of stronger narrative flow and commentary on the results being presented.
At several points, the authors refer to the relative performance of multiple models with a statement similar to "X is much higher than Y, and we have not yet found any explanation". Given the lack of interpretation or understanding why various models perform better or worse than others, how can readers be expected to apply the knowledge presented in this paper to their own datasets or contexts? For instance, are there particular subjects/samples that are driving variation in performance across these models?
-A follow-up to the above point is the surprising result that for some tasks, models without augmentation perform best. Is there any rationale for why this may be the case?
-The definition of the segmentation networks is incomplete until reaching the methods section. It is not clear what model is used here, why it was chosen/constructed, or how different segmentation models may affect the performance and ranking of the synthetic models being compared. Given that the performance on the segmentation task is described and presented as the primary evaluation criteria, these details are important to communicate and rationalize, or compare against alternatives.
-It appears that Table 7 is the critical result of this manuscript, but given the large number of tables and data presented, this is not immediately clear when reading. Also, is there a reason why no rows have been highlighted in this table to identify the best generative models, as was done elsewhere?
-Table 8 seems to present percentages, but the caption describes counts. Harmonize?
-Throughout these results, it is unclear how the sample size for trained models varies across contexts (e.g., Orig + Aug both ticked versus neither ticked), and how that may lead to variations in performance. Please elaborate.

Discussion:
-When discussing the memorization of data through the diffusion model, the authors raise an important point: the initial framing of this manuscript is to use synthetic data for medical image model training to reduce risk and improve the shareability of data/models in clinical contexts. Similar to a point raised above, while the authors may be technically correct that synthetic images not belonging to any one individual would not violate GDPR (though I am no lawyer), it remains that memorized "synthetic" data present a significant concern to security and do violate the spirit of such data sharing policies and restrictions. This concern underscores the validity of the entire approach, and suggests that prior to performing such a comparison for tumor segmentation, the necessary first analysis would be to assess the similarity of synthetic and real data across models using both quantitative and qualitative scoring, and ruling out any generative approaches where clinicians have identified a risk of data memorization.
-The argument of clinical data/samples being treated as a form of public good, and not requiring further consent for use in research or development, is perhaps a slippery slope and many examples exist where a retrospective look identifies the continued use of such data/samples as an unauthorized abuse (perhaps most famously of Henrieta Lacks). I find this perspective a troubling one to present in a work that is chiefly interested in generating synthetic data, as it seems to undermine the objective of ensuring that adequately anonymous data are produced.

Methods:
-Clear and descriptive!

